Interpretable Mesomorphic Networks for Tabular Data

Even though neural networks have been long deployed in applications involving tabular data, still existing neural architectures are not explainable by design. In this paper, we propose a new class of interpretable neural networks for tabular data that are both deep and linear at the same time (i.e. mesomorphic). We optimize deep hypernetworks to generate explainable linear models on a per-instance basis. As a result, our models retain the accuracy of black-box deep networks while offering free-lunch explainability for tabular data by design. Through extensive experiments, we demonstrate that our explainable deep networks have comparable performance to state-of-the-art classifiers on tabular data and outperform current existing methods that are explainable by design.

==> Plots/tsne_global_importance.tex <==
\begin{figure}[t]
      \centering
      \includegraphics[width=0.49\textwidth]{Figures/tsne_education.pdf}
      \includegraphics[width=0.49\textwidth]{Figures/tsne_demographic.pdf}
    \caption[Feature impact comparison]{Feature impact comparison. We compare the impact of one of the most important features, compared to the impact of one of the least important features on the t-SNE embeddings generated from the Census dataset.}
\label{fig:tsne_global_importance}
\end{figure}

==> Plots/xai_explainability.tex <==
\begin{table*}{!tr}{0.5\textwidth}
\centering
\footnotesize
\begin{adjustbox}{width=0.5\textwidth}{
\begin{tabular}{@{}ccccc@{}}
 \toprule
 \textbf{Feature} & \textbf{SHAP} & \textbf{Decision Tree} & \textbf{CatBoost} & \textbf{INN} \\
 \midrule
  Age & 1 & 5 & 3 & 3  \\ 
  Capital Gain & 3 & 4 & 1 & 1 \\ 
  Capital Loss & 9 & 9 & 4 & 4 \\ 
  Education & 5 & 3 & 8 & 9 \\ 
  Gender & 8 & 2 & 9 & 8 \\ 
  Hours per week & 7 & 7 & 6 & 5 \\ 
  Marital Status & 2 & 11 & 5 & 10 \\ 
  Native Country & 11 & 12 & 12 & 12 \\ 
  Occupation & 6 & 6 & 7 & 7 \\ 
  Race & 12 & 10 & 11 & 11 \\
  Relationship & 4 & 1 & 2 & 6 \\
  Work Class & 10 & 8 & 5 & 1 \\
 \bottomrule 
\end{tabular}
}\end{adjustbox}
\caption{The feature rank importances assigned to the Census dataset features by the different methods. A lower rank is associated with a higher feature importance.}
\label{table:xai_explainability}
\vspace{-0.5cm}
\end{table*}


==> Tables/backup_xaibench_result.tex <==
\begin{table}
\caption{Investigating the interpretability of INNs against state-of-the-art interpretability methods. The results are generated on the GaussianLinear dataset with $\rho$ = 0.}
\label{table:gl_interpretability}
\centering
\footnotesize
\begin{adjustbox}{width=1\textwidth}{
\begin{tabular}{@{}llcccccccc@{}}
 \toprule
 \textbf{Dataset} & \textbf{Metric} & \textbf{Random} & \textbf{Breakdown} & \textbf{Maple} & \textbf{LIME} & \textbf{LIMEx} & \textbf{SHAP} & \textbf{B. SHAP} & \textbf{INN}\\
 \midrule
\multirow{5}{*}{Gaussian Linear} & Faithfulness $\left(\uparrow\right)$ & 0.004 & 0.645 & 0.980 & 0.882 & 0.010 & 0.974 & 0.981 &  \textbf{0.987} \\ 
  & Faithfulness (ROAR) $\left(\uparrow\right)$  & -0.039 & 0.494 & 0.548 & 0.544 & 0.049 & 0.549 & 0.550 & \textbf{0.639}  \\ 
  & Infidelity $\left(\downarrow\right)$ & 0.219 & 0.041 & \textbf{0.007}  & \textbf{0.007} & 0.034 & \textbf{0.007}  & \textbf{0.007} & \textbf{0.007}  \\
  & Monotonicity (ROAR) $\left(\uparrow\right)$  & 0.487 & 0.605 & 0.700 & 0.652 & 0.437 & 0.680 & 0.667 & \textbf{0.785}  \\ 
%  Monotonicity & \textbf{0.477} & 0.397 & 0.437 & 0.417 & 0.395 & 0.417 & 0.455 & 0.417  \\ 
%  Shapley & 1.218 & 0.164 & 0.00014 & 0.058 & 0.250 & 0.00115 & \textbf{5.37e-05} & 0.0003  \\ 
  & Shapley Correlation $\left(\uparrow\right)$ & -0.016 & 0.246 & \textbf{0.999} & 0.942 & -0.214 & 0.993 & \textbf{0.999} & \textbf{0.999}  \\ \midrule
\multirow{5}{*}{Gaussian Non-Linear Additive}  & Faithfulness $\left(\uparrow\right)$ & -0.079 & -0.001 & 0.487 & 0.796 & 0.155 & 0.926 & \textbf{0.970} &  0.621 \\ 
  & Faithfulness (ROAR) $\left(\uparrow\right)$  & \textbf{0.05} & 0.006 & 0.04 & -0.04 & -0.060 & -0.01 & -0.036 & 0.027  \\ 
  & Infidelity $\left(\downarrow\right)$ & 0.075 & 0.086 & 0.021 & 0.071 & 0.089 & 0.030  & 0.022 & \textbf{0.018}  \\
  & Monotonicity (ROAR) $\left(\uparrow\right)$  & 0.497 & 0.542 & 0.645 & 0.587 & 0.457 & \textbf{0.67} & 0.632 & 0.637  \\ 
%  Monotonicity & \textbf{0.477} & 0.397 & 0.437 & 0.417 & 0.395 & 0.417 & 0.455 & 0.417  \\ 
%  Shapley & 1.218 & 0.164 & 0.00014 & 0.058 & 0.250 & 0.00115 & \textbf{5.37e-05} & 0.0003  \\ 
  & Shapley Correlation $\left(\uparrow\right)$ & -0.069 & -0.179 & 0.686 & 0.872 & -0.095 & 0.974 & \textbf{0.999} & 0.741  \\ \midrule
  \multirow{5}{*}{Gaussian Piecewise Constant} & Faithfulness $\left(\uparrow\right)$ & 0.091 & 0.634 & 0.967 & 0.929 & 0.016 & 0.981 & \textbf{0.990} &  0.841 \\ 
  & Faithfulness (ROAR) $\left(\uparrow\right)$  & -0.055 & 0.372 & 0.347 & \textbf{0.450} & 0.015 & 0.409 & 0.426 & 0.404  \\ 
  & Infidelity $\left(\downarrow\right)$ & 0.132 & 0.047 & 0.014  & 0.019 & 0.070 & 0.016  & 0.019 & \textbf{0.008}  \\
  & Monotonicity (ROAR) $\left(\uparrow\right)$  & 0.485 & 0.665 & 0.787 & 0.427 & 0.442 & 0.717 & \textbf{0.797} & 0.682  \\ 
%  Monotonicity & \textbf{0.477} & 0.397 & 0.437 & 0.417 & 0.395 & 0.417 & 0.455 & 0.417  \\ 
%  Shapley & 1.218 & 0.164 & 0.00014 & 0.058 & 0.250 & 0.00115 & \textbf{5.37e-05} & 0.0003  \\ 
  & Shapley Correlation $\left(\uparrow\right)$ & -0.078 & 0.099 & 0.983 & 0.959 & 0.157 & 0.991 & \textbf{0.999} & 0.875  \\ \midrule
  Total Wins &  & 1 & 0 & 2 & 2 & 0 & 2 & \textbf{7} & \textbf{7} \\
 \bottomrule 
\end{tabular}
}\end{adjustbox}
\vspace{-0.5cm}
\end{table}









==> Tables/dtree.tex <==
\begin{tabular}{rrrrrrrrr}
\toprule
dataset_id & decision_tree & logistic_regression & random_forest & tabnet & tabresnet & catboost & inn & inn_dtree \\
\midrule
3 & 0.987 & 0.990 & 0.998 & 0.983 & 0.998 & 0.999 & 0.998 & 0.998 \\
12 & 0.938 & 0.999 & 0.998 & 0.995 & 0.999 & 0.999 & 0.999 & 0.999 \\
31 & 0.643 & 0.775 & 0.795 & 0.511 & 0.781 & 0.790 & 0.780 & 0.764 \\
54 & 0.804 & 0.938 & 0.927 & 0.501 & 0.963 & 0.934 & 0.963 & 0.966 \\
1067 & 0.620 & 0.802 & 0.801 & 0.789 & 0.801 & 0.800 & 0.802 & 0.795 \\
1111 & 0.535 & 0.816 & 0.793 & -1.000 & 0.760 & 0.843 & 0.763 & 0.766 \\
1169 & 0.592 & 0.679 & 0.692 & 0.699 & 0.684 & 0.718 & 0.684 & 0.686 \\
1461 & 0.703 & 0.908 & 0.930 & 0.926 & 0.911 & 0.937 & 0.910 & 0.910 \\
1464 & 0.599 & 0.749 & 0.666 & 0.516 & 0.752 & 0.709 & 0.754 & 0.759 \\
1468 & 0.926 & 0.996 & 0.995 & 0.495 & 0.993 & 0.996 & 0.995 & 0.995 \\
1486 & 0.935 & 0.987 & 0.993 & 0.991 & 0.988 & 0.994 & 0.988 & 0.989 \\
1489 & 0.842 & 0.805 & 0.962 & 0.928 & 0.897 & 0.948 & 0.895 & 0.909 \\
1590 & 0.752 & 0.903 & 0.917 & 0.908 & 0.906 & 0.930 & 0.906 & 0.908 \\
1596 & 0.942 & 0.951 & 0.997 & 0.949 & 0.970 & 0.996 & -1.000 & NaN \\
4135 & 0.639 & 0.853 & 0.846 & -1.000 & 0.855 & 0.883 & 0.855 & 0.851 \\
23512 & 0.626 & 0.683 & 0.794 & 0.803 & 0.752 & 0.804 & 0.750 & 0.764 \\
23517 & 0.501 & 0.530 & 0.515 & 0.522 & 0.529 & 0.526 & 0.528 & 0.520 \\
40685 & 0.967 & 0.994 & 1.000 & 0.986 & 1.000 & -1.000 & 0.999 & 0.829 \\
40981 & 0.817 & 0.930 & 0.945 & 0.463 & 0.929 & 0.935 & 0.927 & 0.934 \\
40984 & 0.946 & 0.980 & 0.995 & 0.985 & 0.990 & 0.995 & 0.990 & 0.990 \\
40996 & 0.886 & 0.984 & 0.991 & 0.989 & 0.984 & 0.993 & 0.984 & 0.990 \\
41027 & 0.792 & 0.797 & 0.931 & 0.976 & 0.956 & 0.974 & 0.955 & 0.939 \\
41138 & 0.861 & 0.974 & 0.989 & 0.970 & 0.990 & 0.992 & 0.990 & 0.985 \\
41142 & 0.626 & 0.742 & 0.796 & 0.713 & 0.783 & 0.822 & 0.785 & 0.743 \\
41143 & 0.749 & 0.850 & 0.880 & 0.823 & 0.870 & 0.870 & 0.871 & 0.867 \\
41146 & 0.910 & 0.966 & 0.983 & 0.974 & 0.979 & 0.988 & 0.979 & 0.974 \\
41147 & 0.606 & 0.748 & 0.762 & -1.000 & 0.751 & 0.779 & 0.751 & 0.753 \\
41150 & 0.867 & 0.938 & 0.981 & 0.896 & 0.939 & 0.984 & 0.938 & 0.957 \\
41159 & 0.730 & 0.712 & 0.892 & 0.754 & 0.716 & 0.897 & 0.716 & NaN \\
41161 & 0.857 & 0.995 & 0.999 & 0.997 & 0.998 & 1.000 & 0.998 & NaN \\
41163 & 0.873 & 0.994 & 0.999 & 0.998 & 0.997 & 1.000 & 0.997 & 0.998 \\
41164 & 0.786 & 0.898 & 0.925 & 0.888 & 0.910 & 0.935 & 0.911 & 0.904 \\
41165 & 0.579 & 0.748 & 0.835 & 0.788 & 0.785 & 0.895 & 0.786 & 0.827 \\
41166 & 0.699 & 0.882 & 0.927 & 0.918 & 0.907 & 0.949 & 0.908 & 0.900 \\
41168 & 0.633 & 0.798 & 0.831 & 0.813 & 0.838 & 0.862 & 0.837 & 0.815 \\
41169 & 0.554 & 0.841 & 0.800 & 0.842 & 0.855 & 0.866 & 0.855 & 0.851 \\
\bottomrule
\end{tabular}


==> Text/3-Preliminaries.tex <==
\section{Preliminaries}





==> Text/5-Motivation.tex <==
\section{Motivation}

